Spatial-Filter-Bank-Based Neural Method for Multichannel Speech Enhancement

The performance of deep learning-based multi-channel speech enhancement methods often deteriorates when the geometric parameters of the microphone array change. Traditional approaches to mitigate this issue typically involve training on multiple microphone arrays, which can be costly. To address this challenge, we focus on uniform circular arrays and propose the use of a spatial filter bank to extract features that are approximately invariant to geometric parameters. These features are then processed by a two-stage conformer-based model (TSCBM) to enhance speech quality. Experimental results demonstrate that our proposed method can be trained on a fixed microphone array while maintaining effective performance across uniform circular arrays with unseen geometric configurations during applications.

==> SPL-GNMCSE_ori.tex <==
% \documentclass[journal]{IEEEtran}

% \ifCLASSINFOpdf
% \else
%    \usepackage[dvips]{graphicx}
% \fi
% \usepackage{url}
% \hyphenation{op-tical net-works semi-conduc-tor}
% \usepackage{graphicx}
% \usepackage{color}
% \usepackage{bm}
% \usepackage{float}
% \usepackage{soul}
% \usepackage{xcolor}
% \usepackage{amsmath}
% \usepackage{color}
% \usepackage{bm}
% \usepackage{float}
% \usepackage{tabularx}
% \usepackage{gensymb}
% \usepackage[numbers,sort&compress]{natbib}
% \def\x{{\mathbf x}}
% \def\L{{\cal L}}
% \begin{document}

% \title{Generalized Neural Multichannel Speech Enhancement based on the Implementation of Spatial Filter Banks}

% \author{\it Tianqin Zheng, Jilu Jin, Hanchen Pei, Gongping Huang, Jingdong Chen, and Jacob Benesty}

% \markboth{IEEE SIGNAL PROCESSING LETTERS, VOL. XX, NO. XX, JAN 2025}
% {Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Journals}
% \maketitle

% \begin{abstract}
% The performance of deep learning-based multichannel speech enhancement methods often deteriorates when the geometric parameters of the microphone array change. Traditional approaches to mitigate this issue typically involve training on multiple microphone arrays, which can be costly. To address this challenge, we focus on uniform circular arrays and propose the use of a spatial filter bank to extract features that are approximately invariant to geometric parameters. These features are then processed by a two-stage conformer-based model (TSCBM) to enhance speech quality. Experimental results demonstrate that our proposed method can be trained on a fixed microphone array while maintaining effective performance across uniform circular arrays with unseen geometric configurations during applications. 
% \end{abstract}

% \begin{IEEEkeywords}
% Speech enhancement, multichannel processing, 
% uniform circular microphone arrays, geometry-agnostic.
% \end{IEEEkeywords}


% \IEEEpeerreviewmaketitle


% \section{Introduction}
% \label{sec:intro}
% Speech enhancement techniques focus on improving the quality and clarity of speech signals. Numerous architectures driven by deep learning have emerged for this task~\cite{Tan2018ACR, cao2022cmgan, schroter2022deepfilternet, kim2021se, yu2022dual, fu2019metricgan} and yielded attractive processing results. However, most are designed for single-channel settings, ignoring the essential spatial information in complex settings. Thus, multichannel enhancement methods have been developed~\cite{liu2020multichannel, pop00001, zhang2021adl, casebeer2021nice, 8461639, tolooshams2020channel}, but these typically accommodate only specific microphone array configurations, leading to a degraded performance for unseen array geometry. This limitation arises from the models' inability to adapt to input variations, which result from changes in the array geometry. Thus, achieving model generalization over various arrays is crucial to diminishing the demand for dataset reconstruction and model retraining.


% Some methods have been proposed to improve the adaptability of the model to address the challenge mentioned above \cite{luo2020end, pandey2022tparn, zhang2023toward, lin2024agadir, yoshioka2022vararray}, including applying TAC layers to optimize microphone data integration \cite{luo2020end}, extracting IPD features to acquire spatial information \cite{yoshioka2022vararray}, and building a triple-path network based on spatial self-attention to process array observations \cite{pandey2022tparn}. Although these methods are effective, they face notable restrictions: they all require separate processing for each channel, which leads to high computational overhead, and they rely on diverse datasets for generalization, which is not feasible for real-world implementations.


% To address these challenges, we aim to train a model on a fixed array to ensure robust performance across diverse geometries, with a focus on UCAs. We propose a spatial filter bank for feature extraction that is nearly invariant to geometric changes. Using a model based on~\cite{cao2022cmgan}, we process these characteristics to enhance the speech signal, reducing computational complexity through joint channel processing. Experiments reveal that our method exceeds existing approaches and maintains performance on unseen arrays.

% \textcolor{blue}{Our contributions to multichannel speech enhancement are multifaceted. First, we identify key factors that impact model performance across diverse microphone arrays and develop an interpretable feature extraction method to maintain top performance. Second, the proposed method is broadly applicable and can integrate with multiple multichannel speech enhancement models to enhance their generalization to unseen arrays. Third, although our study mainly addresses UCAs for simplicity, the feature extraction method is extendable to planar arrays with arbitrary geometry, as mentioned in \cite{huangarbitrary}.}


% \section{Signal Model and Problem Formulation}
% \label{sec:signal model}

% Consider a UCA consisting of $M$ omnidirectional sensors uniformly spaced around a circle of radius $r$.  Taking the center of the UCA as the reference point and assuming a plane wave arriving from an azimuth angle $\theta$, the phase delay at the $m$th sensor relative to the reference can be expressed as $\zeta_m \left( \omega, \theta \right) = e^{\jmath \overline{\omega} \cos \left( \theta - \psi_m \right)}$, $m = 1, 2, \ldots, M$, where $\jmath$ is the imaginary unit, $\overline{\omega} = \omega r / c$, $\omega$ is the angular frequency, and $c$ denotes the speed of sound in air. The steering vector can then be represented as
% \begin{align}
%     \label{sv}
%     \mathbf{d} \left( \omega, \theta \right)
%     & = \left[ \begin{array}{cccc}
%     \zeta_1 \left( \omega, \theta \right) & \zeta_2 \left( \omega, \theta \right) & \cdots & \zeta_M \left( \omega, \theta \right)
%     \end{array}\right]^T.
% \end{align}
% In the short-time-Fourier-transform (STFT) domain, the signals received by the UCA can be written as
% \begin{align}
%     \label{y-vect-def}
%     \mathbf{y} \left( k,\omega \right)
%     & = \left[ \begin{array}{cccc}
%     Y_1 \left( k, \omega \right) & Y_2 \left( k, \omega \right) & \cdots & Y_M \left( k, \omega \right)
%     \end{array} \right]^T \nonumber \\
%     & = \mathbf{x}_\mathrm{d} \left( k, \omega \right) + \mathbf{v} \left( k, \omega \right),
% \end{align}
% where $\mathbf{v} \left( k,\omega \right)$ of length $M$ denotes the vector of background noise, and
% \begin{align}
%     \label{x-d-vect-def}
%     \mathbf{x}_\mathrm{d} \left( k, \omega \right)
%     & = \left[ \begin{array}{ccc}
%     X_{1, \mathrm{d}} \left( k, \omega \right) & \cdots & X_{M, \mathrm{d}} \left( k, \omega \right)
%     \end{array} \right]^T
% \end{align}
% also of length $M$ represents the desired signal originated from the source of interest,  with (see Subsection~\ref{ssec:SFE} for more details)
% \begin{align}
%     \label{x-d-def}
%     X_\mathrm{d} \left( k, \omega \right)
%     & = G \left( \omega \right) S \left( k, \omega \right),
% \end{align}
% $G \left( \omega \right)$ being the transfer function corresponding to the direct path and early reflections,  and $S \left( k, \omega \right)$ denoting the source signal.

% The objective of this work is to estimate $X_\mathrm{d} \left( k, \omega \right)$ from the array observations $\mathbf{y} \left( k, \omega \right)$. To accomplish this, we derive a neural network (NN) based method.

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.475\textwidth]{Fig1-ver3.pdf} 
%     \caption{The overall architecture of the proposed TSCBM+FB.}
%     \label{fig:whole}
% \end{figure}


% \section{Method Derivation}
% \label{sec:method}

% To address the performance degradation of trained models on previously unseen arrays, we introduce a method called TSCBM+FB, which stands for two-stage conformer-based model (TSCBM) with filter bank (FB). This approach first extracts features that are independent of the array radius and the number of microphones using a spatial FB. These features are then processed and enhanced by the TSCBM. The overall architecture of this model is illustrated in Fig.~\ref{fig:whole}. In the following subsections, we detail the feature extraction process and provide a comprehensive explanation of the TSCBM architecture.

% \subsection{Spatial Feature Extraction}
% \label{ssec:SFE}

% Given the nature of sound propagation, the transfer function $G \left( \omega \right)$ is composed of contributions from both the direct and multiple reflection paths; consequently, $G \left( \omega \right)$ can be expressed as follows:
% \begin{align}
%     \label{g-fact}
%     G \left( \omega \right)
%     & = \sum^L_{l = 1} Q_l \left( \omega \right) ,
% \end{align}
% where $Q_l \left( \omega \right)$ represents the transfer function of the $l$th path with $L$ being the total number of paths. The desired component of the source signal received by the $m$th microphone can then be written as
% \begin{align}
%     \label{x-m-d-fact}
%     X_{m, \mathrm{d}} \left( k, \omega \right)
%     & = \sum^L_{l = 1} Q_l \left( \omega \right) \zeta_m \left( \omega, \theta_l \right) S \left( k, \omega \right),
% \end{align}
% where $\zeta_m \left( \omega, \theta_l \right)$ denotes the phase delay of the $l$th path to the $m$th microphone. The vector $\mathbf{x}_\mathrm{d} \left( k, \omega \right)$ can then be expressed as
% \begin{align}
%     \label{x-d-vect-def-2}
%     \mathbf{x}_\mathrm{d} \left( k, \omega \right)
%     & = \sum^L_{l = 1} Q_l \left( \omega \right) S \left( k, \omega \right) \mathbf{d} \left( \omega, \theta_l \right).
% \end{align}
% As indicated by \eqref{x-d-vect-def-2}, changes in the UCA geometry, such as changes in the number of sensors or the radius, will affect $\mathbf{d} \left( \omega, \theta_l \right)$. This, in turn, can lead to performance degradation in deep learning models. Therefore, it is crucial to extract features that are independent of the array geometry. Specifically, a spatial filter can be used to achieve this. Given a spatial filter $\mathbf{h} \left( \omega \right)$, the filtered signal is
% \begin{align}
%     \label{z-def}
%     Z \left( k, \omega \right)
%     & = \mathbf{h}^H \left( \omega \right) \mathbf{y} \left( k, \omega \right) \nonumber \\
%     & = \mathbf{h}^H \left( \omega \right) \mathbf{x}_\mathrm{d} \left( k, \omega \right) + \mathbf{h}^H \left( \omega \right) \mathbf{v} \left( k, \omega \right) \nonumber \\
%     & = X_\mathrm{fd} \left( k, \omega \right) + V_\mathrm{rn} \left( k, \omega \right),
% \end{align}
% where the superscript $^H$ is the conjugate-transpose operator, $X_\mathrm{fd} \left( k, \omega \right)$ is the filtered desired signal, and $V_\mathrm{rn} \left( k, \omega \right)$ is the residual noise. 

% Let us examine the structure of $X_\mathrm{fd} \left( k, \omega \right)$, which is
% \begin{align}
%     \label{x-fd-def}
%     X_\mathrm{fd} \left( k, \omega \right)
%     & = \sum^L_{l = 1} Q_l \left( \omega \right) S \left( k, \omega \right) \mathbf{h}^H \left( \omega \right) \mathbf{d} \left( \omega, \theta_l \right) \nonumber \\
%     & = \sum^L_{l = 1} Q_l \left( \omega \right) S \left( k, \omega \right) \mathcal{B} \left[ \mathbf{h} \left( \omega \right), \theta_l \right],
% \end{align}
% where $\mathcal{B} \left[ \mathbf{h} \left( \omega \right), \theta_l \right]$ denotes the spatial response, i.e., the beampattern at azimuth angle $\theta_l$. 
% As shown in \eqref{x-fd-def}, $Q_l \left( \omega \right)$ and $S \left( k, \omega \right)$ are not dependent on the array geometry. If the spatial response $\mathcal{B} \left[ \mathbf{h} \left( \omega \right), \theta_l \right]$ of the spatial filter is independent of the geometry of the UCA, then the extracted speech feature will also be independent of the geometric parameters.

% To ensure that the beampattern remains independent of geometric parameters, we can design the filter to approximate the desired directivity pattern. To achieve this, we employ the method proposed in~\cite{huang2017design}. For a UCA, the ideal beampattern with the mainlobe directed towards $\theta_\mathrm{s}$ can be expressed as
% \begin{align}
%     \mathcal{B} \left( \mathbf{b}_{N}, \theta \right)
%     & = \sum_{n=-N}^N b_{N,n} e^{\jmath n \left( \theta - \theta_\mathrm{s} \right)} \nonumber \\
%     & = \mathbf{b}_N^T \mathbf{p} \left( \theta \right),
% \end{align}
% where $\mathbf{b}_N$ contains the coefficients determining the shape of the ideal beampattern, $N$ is the order of the beampattern, and 
% \begin{align}
%     \mathbf{p} \left( \theta \right)
%     & = \left[\begin{array}{ccccc}
%     e^{-\jmath N \theta} & \cdots & 1 & \cdots & e^{\jmath N \theta}
%     \end{array} \right]^T.
% \end{align}
% The design of the beamforming filter can be approached from a least-squares perspective \cite{huang2017design}. The filter is formulated as follows:
% \begin{align}
%     \label{h-vect-def}
%     \mathbf{h} \left( \omega \right)
%     & = \frac{1}{M} \mathbf{\Psi}^H \mathbf{J}^* \left( \overline{\omega} \right) \mathbf{\Upsilon}^* \left( \theta_{\mathrm{s}} \right) \mathbf{b}_N,
% \end{align}
% where the superscript $^*$ is the conjugate operator, and
% \begin{align}
%     \mathbf{\Psi}
%     & = \left[ \begin{array}{ccccc}
%     \boldsymbol{\psi}_{-N}^* & \cdots & \boldsymbol{\psi}_0^* & \cdots & \bm{\psi}_N^*
%     \end{array} \right]^T, \\
%     \boldsymbol{\psi}_n
%     & = \left[ \begin{array}{cccc}
%     e^{-\jmath n \psi_1} & e^{-\jmath n \psi_2} & \cdots & e^{-\jmath n \psi_M}
%     \end{array} \right]^T, \\
%     \mathbf{J} \left( \overline{\omega} \right)
%     & = \mathrm{diag} \left[ \frac{1}{\jmath^{-N}J_{-N} \left( \overline{\omega} \right)} \cdots \frac{1}{J_0 \left( \overline{\omega} \right)} \cdots \frac{1}{\jmath^N J_N \left( \overline{\omega} \right)} \right], \\
%     \mathbf{\Upsilon} \left( \theta_\mathrm{s} \right)
%     & = \mathrm{diag} \left[ e^{\jmath N \theta_\mathrm{s}} ~~\cdots~~ 1 ~~\cdots~~ e^{-\jmath N \theta_\mathrm{s}} \right],
% \end{align}
% with $J_n \left( \cdot \right)$ being the $n$th order Bessel function of the first kind. 

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.4\textwidth]{Fig2.eps} \vskip -12pt
% \caption{Designed second-order supercardioid beampattern with varying UCA geometric parameters. Conditions: $\theta_\mathrm{s} = 0^\circ$ and $f = 4$~kHz.}
% \label{fig:beampattern1}
% \end{figure}

% Figure~\ref{fig:beampattern1} shows the beampatterns of a supercardioid beamformer designed for a UCA with different geometric parameters. The beampatterns are highly consistent, demonstrating that they remain largely unaffected by geometric variations. This consistency highlights that the features extracted using this method are primarily independent of geometric parameters, which is crucial for maintaining robustness across various array configurations.



% Although the beampattern of a spatial filter can be designed to be independent of the geometric parameters of the UCA, it mainly enhances sound from a specific direction, $\theta_\mathrm{s}$, while attenuating sound from other directions, as shown in Fig.~\ref{fig:beampattern1}. Since the speaker’s location is typically unknown in practice, it is necessary to use a set of spatial filters oriented in different directions to form a spatial FB for feature extraction. Specifically, we use a total of $I$ filters, where the $i$th filter orients toward $\theta_\mathrm{s} = \frac{i}{I} 2\pi$, and the output from this filter is denoted as $Z_i$.


% \subsection{Model Architecture}

% \textcolor{blue}{Our network is built on CMGAN \cite{cao2022cmgan}, which features a well-known dual-path architecture that effectively captures temporal and frequency information in speech signals and demonstrates impressive performance in speech enhancement tasks. To address the specific challenges we faced, we simplified the network structure and adapted the proposed approach to the TSCBM. It is important to note that our methodology extends beyond TSCBM and is applicable to most multichannel speech enhancement models. We select TSCBM as the backbone model to simultaneously process multichannel signals and avoid separately processing signals in individual channels \cite{luo2020end, pandey2022tparn, yoshioka2022vararray}, which is essential for reducing computational complexity.}

% \subsubsection{Input Features}
% The spatial FB's output features are compressed to equalize the significance of softer sounds against louder ones:
% \begin{align} 
% Z_i^{'} = |Z_i|^c e^{\jmath \angle{Z_i}},
% \end{align}
% where $Z_i^{'}$ is the compressed feature and $c=0.3$ is the compression exponent as per \cite{cao2022cmgan}. The real and imaginary parts of $Z_i^{'}$ are concatenated to form the input $Z^{'} \in \mathcal{R}^{B \times 2I \times T \times F}$, with $T$ and $F$ representing time and frequency dimensions, respectively.

% \subsubsection{Encoder}
% The encoder maps $Z^{'}$ into a latent feature space. It initiates with a convolutional block with a kernel of $(1,1)$ and stride $(1,1)$, followed by instance normalization and PReLU activation. This yields an intermediate feature map $[B,C,T,F]$ with $C=64$. A dilated DenseNet with dilation factors of 1 and 2 is then applied. The process ends with a convolutional block with a kernel of $(1,3)$ and stride $(1,2)$, downsampling the frequency dimension.

% \subsubsection{TSCB Block}
% Intermediate features pass through two-stage conformer blocks (TSCBs) to capture temporal and frequency dependencies. Each TSCB, as shown in Fig.~\ref{fig:whole}(b), contains two conformer blocks, each addressing temporal and frequency dependencies. These blocks include two FFNNs, an MHSA mechanism with four heads, and a convolution module. Skip connections are used to preserve feature integrity.

% \subsubsection{Decoder}
% The decoder reconstructs the desired signal spectrum. It begins with a dilated DenseNet mirroring the encoder's architecture. A sub-pixel convolution block follows, doubling the feature dimension to $C=128$ and upsampling the frequency dimension via pixel shuffle. The final convolution block includes instance normalization, PReLU activation, and a kernel of $(1,2)$, yielding a final feature map with $C=2$ for the real and imaginary parts of the signal spectrum.




% \section{Experiments}
% \label{sec:exp}
% \vspace{10pt}
% \subsection{Experimental Setup}
% \vspace{10pt}
% \subsubsection{Dataset}
% We simulated a multichannel dataset using the VoiceBank and DEMAND datasets. The training set features clean speech mixed with 12 types of background noise from DEMAND at SNR levels ranging from $-5$ to $10$~dB. The test set introduces 5 new noise types from DEMAND, with multichannel RIR generated via the Image model. Room dimensions vary from $3$~m $\times$ $3$~m $\times$ $2.5$~m to $7$~m $\times$ $9$~m $\times$ $3$~m, and reverberation time ($T_{60}$) is randomly set between $0.2$ and $0.35$ seconds. Microphone array, sound source, and noise source positions are randomly determined, with a minimum directional angle difference of $5^\circ$ between the target speech and interference. To test generalization across microphone array geometries, the number of microphones and UCA radius differ between training (5 microphones, 0.5~cm radius) and test sets (7 or 9 microphones, 1~cm or 1.5~cm radius). Unlike most related work that trains on multiple arrays for generalizability, our approach trains on a single UCA type and evaluates performance across four distinct UCA types.

% % {\color{red} What is CSIG, CBAK, COVL?}

% % {\color{blue}
% Evaluation metrics include Floating Point Operations Per Second(FLOPS) of the model, perceptual evaluation of speech quality (PESQ)~\cite{pesq},
% mean opinion score (MOS) predictions of speech distortion (CSIG), MOS predictions of intrusiveness of background noise (CBAK), MOS predictions of overall processed speech quality (COVL)~\cite{csigxx}, and STOI~\cite{stoi}. PESQ ranges from $-0.5$ to $4.5$, CSIG, CBAK, and COVL from $1$ to $5$, and STOI from $0$ to $1$. Apart from FLOPS, higher scores on all other metrics indicate better performance.
% % }

% \subsubsection{Training Configuration}
% The training set utterances are truncated into $2$-second segments, while the test set uses full-length sentences. Following the method outlined in~\cite{cao2022cmgan}, we apply a Hamming window with a $25$-ms window length ( corresponding to 400-point FFT) and a hop size of $6.25$ ms (i.e., $75\%$ overlap).
% A total of 9, (i.e., $I=9$) spatial filters are used, which are oriented at $\theta_\mathrm{s} = \frac{i}{I} 2 \pi$ to extract $I$ features, employing a second-order supercardioid filter. The coefficients for the ideal beampattern used to design this filter are $\mathbf{b}_N = \left[0.1035, 0.242, 0.309, 0.242, 0.1035\right]^T$.
% The loss function is based on the mean-squared error of the real part, imaginary part, and magnitude of the estimated spectrum. During training, the AdamW optimizer~\cite{loshchilov2017decoupled} is employed with a learning rate of $5 \times 10^{-4}$.

% \subsubsection{Comparison Methods}
% For comparison, we employ the FaSNet+TAC network~\cite{luo2020end} as a baseline. Originally designed for permutation- and number-invariant speech separation, it is modified for speech enhancement by omitting the beamforming component due to the absence of a reference center microphone. This modified model is termed DPRNN+TAC. \textcolor{blue}{Additionally, we introduce the DPRNN+FB model, which is a variant of DPRNN+TAC without the TAC module, allowing joint channel processing. It is then integrated with our feature extraction method to demonstrate that our approach can circumvent the high computational complexity associated with TAC-like modules in array geometry-agnostic tasks.} To address the degradation of deep learning models on unseen UCAs, we train TSCBM on a fixed array with 5 microphones and a radius $0.5$~cm. For testing, if the test array exceeds 5 microphones, we select $5$ with azimuth angles closest to the training array as the TSCBM input, referred to as TSCBM+select. Our proposed method, incorporating spatial FB, is dubbed TSCBM+FB.

% \subsection{Experimental Results}
% \begin{table}[htbp]
% \centering
%  \caption{Speech enhancement performance of the DPRNN+TAC, TSCBM+select, and  TSCBM+FB methods.}
%  \renewcommand{\arraystretch}{1.2}
%  % \vspace{5pt}
% \scalebox{1}{
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{lcccccc} 
% \hline
% Model     &FLOPS   & PESQ          & CSIG          & CBAK          & COVL          & STOI           \\ \hline
% Noisy      &\ & 1.23          & 2.72          & 1.86          & 1.99          & 0.789           \\ \hline
% DPRNN+TAC  &31.3G    & 2.25          & 4.09          & 3.06          & 3.23          & 0.914          \\
% TSCBM+select &28.3G    & 2.50          & 4.02          & 3.21          & 3.32          & 0.934          \\
% DPRNN+FB &\textbf{2.77G}     &2.25 &4.15 &2.98 &3.26 &0.911\\
% TSCBM+FB    &28.3G    &\textbf{2.76} & \textbf{4.36} & \textbf{3.30} & \textbf{3.64} & \textbf{0.947} \\ 
% \hline
% \end{tabular}}
% \label{tab:table1}
% \end{table}
% %\subsubsection{Superior performance of TSCBM+FB}
% We first evaluate the performance of these methods on the test set. The results are detailed presented in Table~\ref{tab:table1}. The results indicate that TSCBM+FB excels when our feature extraction methods are employed, underscoring the model's ability to adapt to unseen microphone arrays by extracting geometry-independent features. \textcolor{blue}{Notably, DPRNN+FB and DPRNN+TAC show comparable performance, despite DPRNN+FB's computational complexity being roughly one-tenth of DPRNN+TAC's. This suggests that our feature extraction methods can significantly reduce computational demands in tasks agnostic to array geometry.} Furthermore, TSCBM+select outperforms DPRNN+TAC, validating the effectiveness of selecting microphones similar to those used in training. 

% % And the huge performance increase from DPRNN+TAC and DPRNN+TAC+FB also shows that the feature extracting methods can be applied to other multichannel speech enhancement models and improve their performance in unseen arrays. In particular, with less computation complexity, the performance of our proposed method is very close to DPRNN+TAC+FB, showing that with our feature extraction method, The gains achieved by employing the TAC module are primarily attributed to the increase in computational complexity; similar effects can be achieved with other methods that have comparable computational complexity.


% %\subsubsection{Portability of spatial filter bank}
% % We then compare the performance of the models with and without the spatial FB, as shown in Table~\ref{tab:table2}. The results clearly indicate that incorporating the spatial FB into the DPRNN+TAC model leads to a significant performance improvement. This illustrates that our proposed method integrates seamlessly with other deep learning models, enhancing their ability to generalize across different microphone array geometries and improving overall performance.

% % \begin{table}[t!]
% % \centering
% % \caption{Speech enhancement performance of the DPRNN+TAC and DPRNN+TAC+FB  methods.}
% % \vspace{10pt}
% % \renewcommand{\arraystretch}{1.2}
% % \scalebox{0.85}{\begin{tabular}{lccccl}
% % \hline
% % Model        & PESQ & CSIG & CBAK & COVL & STOI \\ \hline
% % DPRNN+TAC    & 2.25      & 4.09       & 3.06       & 3.23       & 0.914      \\
% % DPRNN+TAC+FB & 2.79      & 4.49      & 3.26      & 3.72      & 0.948      \\ \hline
% % \end{tabular}}
% % \label{tab:table2}
% % \end{table}
% \begin{figure}[t!]
% 	\centering
% 	\begin{minipage}{0.48\linewidth}
% 		\centering
% 		\includegraphics[width=0.9\linewidth]{Fig3-pesq.eps}
% 		% \caption{chutian1}
% 		% \label{chutian1}%文中引用该图片代号
% 	\end{minipage}
% 	\begin{minipage}{0.48\linewidth}
% 		\centering
% 		\includegraphics[width=0.9\linewidth]{Fig3-csig.eps}
% 		% \caption{chutian2}
% 		% \label{chutian2}%文中引用该图片代号
% 	\end{minipage}
% 	%\qquad
% 	%让图片换行，
	
% 	\begin{minipage}{0.48\linewidth}
% 		\centering
% 		\includegraphics[width=0.9\linewidth]{Fig3-cbak.eps}
% 		% \caption{chutian3}
% 		% \label{chutian3}%文中引用该图片代号
% 	\end{minipage}
% 	\begin{minipage}{0.48\linewidth}
% 		\centering
% 		\includegraphics[width=0.9\linewidth]{Fig3-covl.eps}
% 		% \caption{chutian4}
% 		% \label{chutian4}%文中引用该图片代号
% 	\end{minipage} \vskip -6pt 
%  \caption{Performance comparison between DPRNN+TAC and TSCBM+FB versus different numbers of microphones and radii: (a)~PESQ, (b)~CSIG, (c)~CBAK, and (d)~COVL.}
%  \label{fig:fig3}
% \end{figure}
 
% %\subsubsection{Generalization Ability}
% To evaluate the generalization of our method across microphone array geometries, we create 9 test sets with varying radii (0.5, 1, and 1.5 cm) and microphone counts (5, 7, and 9). Both DPRNN+TAC and TSCBM+FB are trained on a UCA with 5 microphones and a 0.5 cm radius. The test set configuration ($M=5$, $r=0.5$~cm) matches the training set, serving as a "reference performance." Figure~\ref{fig:fig3} displays the performance metrics. DPRNN+TAC maintains consistent performance across different microphone numbers but degrades with changes in array radius, as the TAC module handles channel count variations but not radius changes. In contrast, TSCBM+FB shows stable performance across both radius and microphone count variations, indicating its robust generalization across array geometries.



% \section{Conclusions}
% \label{sec:conclusion}
% \textcolor{blue}{This paper tackles the challenge of training a model on a fixed uniform circular microphone array to maintain consistent performance across diverse UCAs. We utilize a spatial FB to extract geometry-independent features for speech enhancement via TSCBM. Despite its simplicity, our feature extraction method proves highly effective. Our method demonstrates robust performance and generalization across array geometries. While focusing on circular arrays for simplicity, the principles apply to arbitrary-shaped planar arrays, positioning our approach as a potential standard for generalizing across various microphone configurations. Future work will explore the method's impact on arbitrary-shaped microphone arrays.}

% % References should be produced using the bibtex program from suitable
% % BiBTeX files (here: strings, refs, manuals). The IEEEbib.bst bibliography
% % style file from IEEE produces unsorted bibliography list.
% % -------------------------------------------------------------------------
% % \vfill\pagebreak


% \footnotesize

% \begin{thebibliography}{10}

% \bibitem{Tan2018ACR}
% K.~Tan and D.~Wang, ``{A convolutional recurrent neural network for real-time
%   speech enhancement},'' in {\em Proc. Interspeech}, 2018.

% \bibitem{cao2022cmgan}
% S.~Abdulatif, R.~Cao, and B.~Yang, ``{CMGAN: conformer-based Metric-GAN for
%   monaural speech enhancement},'' {\em IEEE/ACM Trans. Audio, Speech, Lang.
%   Process.}, vol.~32, pp.~2477--2493, 2024.

% \bibitem{schroter2022deepfilternet}
% H.~Schroter, A.~N. Escalante-B, T.~Rosenkranz, and A.~Maier, ``{DeepFilterNet:
%   a low complexity speech enhancement framework for full-band audio based on
%   deep filtering},'' in {\em Proc. IEEE ICASSP}, pp.~7407--7411, 2022.

% \bibitem{kim2021se}
% E.~Kim and H.~Seo, ``{S{E}-{C}onformer: time-domain speech enhancement using
%   Conformer.},'' in {\em Proc. Interspeech}, pp.~2736--2740, 2021.

% \bibitem{yu2022dual}
% G.~Yu, A.~Li, C.~Zheng, Y.~Guo, Y.~Wang, and H.~Wang, ``{Dual-branch
%   attention-in-attention transformer for single-channel speech enhancement},''
%   in {\em Proc. IEEE ICASSP}, pp.~7847--7851, 2022.

% \bibitem{fu2019metricgan}
% S.-W. Fu, C.-F. Liao, Y.~Tsao, and S.-D. Lin, ``{M}etric{GAN}: generative
%   adversarial networks based black-box metric scores optimization for speech
%   enhancement,'' in {\em Proceedings of the 36th International Conference on
%   Machine Learning} (K.~Chaudhuri and R.~Salakhutdinov, eds.), vol.~97 of {\em
%   Proceedings of Machine Learning Research}, pp.~2031--2041, 09--15 Jun 2019.

% \bibitem{xx}
% G.~Li, S.~Liang, S.~Nie, W.~Liu, M.~Yu, L.~Chen, S.~Peng, and C.~Li,
%   ``{Direction-aware speaker beam for multi-channel speaker extraction},'' in
%   {\em Proc. Interspeech}, pp.~2713--2717, 2019.

% \bibitem{liu2020multichannel}
% C.-L. Liu, S.-W. Fu, Y.-J. Li, J.-W. Huang, H.-M. Wang, and Y.~Tsao,
%   ``{Multichannel speech enhancement by raw waveform-mapping using fully
%   convolutional networks},'' {\em IEEE/ACM Trans. Audio, Speech, Lang.
%   Process.}, vol.~28, pp.~1888--1900, Feb 2020.

% \bibitem{pop00001}
% Z.-Q. Wang, P.~Wang, and D.~Wang, ``{Complex spectral mapping for single- and
%   multi-channel speech enhancement and robust ASR},'' {\em IEEE/ACM Trans.
%   Audio, Speech, Lang. Process.}, vol.~28, pp.~1778--1787, May 2020.

% \bibitem{zhang2021adl}
% Z.~Zhang, Y.~Xu, M.~Yu, S.-X. Zhang, L.~Chen, and D.~Yu, ``{ADL-MVDR: all deep
%   learning MVDR beamformer for target speech separation},'' in {\em Proc. IEEE
%   ICASSP}, pp.~6089--6093, 2021.

% \bibitem{casebeer2021nice}
% J.~Casebeer, J.~Donley, D.~Wong, B.~Xu, and A.~Kumar, ``{NICE-Beam: neural
%   integrated covariance estimators for time-varying beamformers},'' {\em arXiv
%   preprint arXiv:2112.04613}, 2021.

% \bibitem{8461639}
% Z.-Q. Wang, J.~Le~Roux, and J.~R. Hershey, ``{Multi-channel deep clustering:
%   discriminative spectral and spatial embeddings for speaker-independent speech
%   separation},'' in {\em Proc. IEEE ICASSP}, pp.~1--5, 2018.

% \bibitem{tolooshams2020channel}
% B.~Tolooshams, R.~Giri, A.~H. Song, U.~Isik, and A.~Krishnaswamy,
%   ``{Channel-attention dense U-Net for multichannel speech enhancement},'' in
%   {\em ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and
%   Signal Processing (ICASSP)}, pp.~836--840, 2020.

% \bibitem{luo2020end}
% Y.~Luo, Z.~Chen, N.~Mesgarani, and T.~Yoshioka, ``{End-to-end microphone
%   permutation and number invariant multi-channel speech separation},'' in {\em
%   Proc. IEEE ICASSP}, pp.~6394--6398, 2020.

% \bibitem{pandey2022tparn}
% A.~Pandey, B.~Xu, A.~Kumar, J.~Donley, P.~Calamia, and D.~Wang, ``{TPARN:
%   triple-path attentive recurrent network for time-domain multichannel speech
%   enhancement},'' in {\em Proc. IEEE ICASSP}, pp.~6497--6501, 2022.

% \bibitem{zhang2023toward}
% W.~Zhang, K.~Saijo, Z.-Q. Wang, S.~Watanabe, and Y.~Qian, ``{Toward universal
%   speech enhancement for diverse input conditions},'' in {\em 2023 IEEE
%   Automatic Speech Recognition and Understanding Workshop (ASRU)}, pp.~1--6,
%   2023.

% \bibitem{lin2024agadir}
% J.~Lin, N.~Moritz, Y.~Huang, R.~Xie, M.~Sun, C.~Fuegen, and F.~Seide,
%   ``{AGADIR: towards array-geometry agnostic directional speech recognition},''
%   in {\em Proc. IEEE ICASSP}, pp.~11951--11955, 2024.

% \bibitem{yoshioka2022vararray}
% T.~Yoshioka, X.~Wang, D.~Wang, M.~Tang, Z.~Zhu, Z.~Chen, and N.~Kanda,
%   ``{VarArray: array-geometry-agnostic continuous speech separation},'' in {\em
%   Proc. IEEE ICASSP}, pp.~6027--6031, 2022.

% \bibitem{huang2017design}
% G.~Huang, J.~Benesty, and J.~Chen, ``{On the design of frequency-invariant
%   beampatterns with uniform circular microphone arrays},'' {\em IEEE Trans.
%   Audio, Speech, Lang. Process.}, vol.~25, pp.~1140--1153, May 2017.

% \bibitem{ulyanov2016instance}
% D.~Ulyanov, A.~Vedaldi, and V.~Lempitsky, ``{Instance normalization: the
%   missing ingredient for fast stylization},'' {\em arXiv preprint
%   arXiv:1607.08022}, 2016.

% \bibitem{he2015delving}
% K.~He, X.~Zhang, S.~Ren, and J.~Sun, ``{Delving deep into Rectifiers:
%   surpassing human-level performance on ImageNet classification},'' in {\em
%   Proceedings of the IEEE international conference on computer vision},
%   pp.~1026--1034, 2015.

% \bibitem{pandey2020densely}
% A.~Pandey and D.~Wang, ``Densely connected neural network with dilated
%   convolutions for real-time speech enhancement in the time domain,'' in {\em
%   Proc. IEEE ICASSP}, pp.~6629--6633, 2020.

% \bibitem{gulati2020conformer}
% A.~Gulati, J.~Qin, C.-C. Chiu, N.~Parmar, Y.~Zhang, J.~Yu, W.~Han, S.~Wang,
%   Z.~Zhang, Y.~Wu, {\em et~al.}, ``{Conformer: convolution-augmented
%   transformer for speech recognition},'' {\em Proc. Interspeech},
%   2020.

% \bibitem{voicebank}
% C.~Veaux, J.~Yamagishi, and S.~King, ``{The voice bank corpus: design,
%   collection and data analysis of a large regional accent speech database},''
%   in {\em 2013 International Conference Oriental COCOSDA held jointly with 2013
%   Conference on Asian Spoken Language Research and Evaluation
%   (O-COCOSDA/CASLRE)}, pp.~1--4, 2013.

% \bibitem{thiemann2013diverse}
% J.~Thiemann, N.~Ito, and E.~Vincent, ``{The diverse environments multi-channel
%   acoustic noise database (DEMAND): A database of multichannel environmental
%   noise recordings},'' in {\em Proceedings of Meetings on Acoustics}, vol.~19,
%   2013.

% \bibitem{allen1979image}
% J.~B. Allen and D.~A. Berkley, ``Image method for efficiently simulating
%   small-room acoustics,'' {\em J. Acoust. Soc. Am.}, vol.~65, no.~4,
%   pp.~943--950, 1979.

% \bibitem{pesq}
% A.~Rix, J.~Beerends, M.~Hollier, and A.~Hekstra, ``{Perceptual evaluation of
%   speech quality (PESQ)-a new method for speech quality assessment of telephone
%   networks and codecs},'' in {\em Proc. IEEE ICASSP}, vol.~2, pp.~749--752
%   vol.2, 2001.

% \bibitem{csigxx}
% Y.~Hu and P.~C. Loizou, ``Evaluation of objective quality measures for speech
%   enhancement,'' {\em IEEE/ACM Trans. Audio, Speech, Lang. Process.}, vol.~16,
%   pp.~229--238, Jan 2008.

% \bibitem{stoi}
% C.~H. Taal, R.~C. Hendriks, R.~Heusdens, and J.~Jensen, ``A short-time
%   objective intelligibility measure for time-frequency weighted noisy speech,''
%   in {\em Proc. IEEE ICASSP}, pp.~4214--4217, 2010.

% \bibitem{loshchilov2017decoupled}
% I.~Loshchilov and F.~Hutter, ``{Decoupled weight decay regularization},'' {\em
%   arXiv preprint arXiv:1711.05101}, 2017.

% \bibitem{huangarbitrary}
% G.~Huang, J.~Chen, and J.~Benesty, ``{On the design of differential beamformers with arbitrary planar microphone array geometry},'' {\em JASA}, vol.~144, pp.~EL66--EL70, 2018

% % @article{huang2018design,
% %   title={On the design of differential beamformers with arbitrary planar microphone array geometry},
% %   author={Huang, Gongping and Chen, Jingdong and Benesty, Jacob},
% %   journal={The Journal of the Acoustical Society of America},
% %   volume={144},
% %   number={1},
% %   pages={EL66--EL70},
% %   year={2018},
% %   publisher={AIP Publishing}
% % }
% \end{thebibliography}


% \end{document}


==> formular.tex <==
% \documentclass[journal]{IEEEtran}

% \ifCLASSINFOpdf
% \else
%    \usepackage[dvips]{graphicx}
% \fi
% \usepackage{url}
% \usepackage{graphicx}
% \usepackage{color}
% \usepackage{bm}
% \usepackage{float}
% \usepackage{soul}
% \usepackage{xcolor}
% \usepackage{amsmath}
% \usepackage{color}
% \usepackage{bm}
% \usepackage{float}
% \usepackage{tabularx}
% \usepackage{gensymb}
% \def\x{{\mathbf x}}
% \def\L{{\cal L}}
% \begin{document}

% \title{Spatial-Filter-Bank-Based Neural Method for Multichannel Speech Enhancement}

% \author{\it Tianqin Zheng, Jilu Jin, Hanchen Pei, Gongping Huang, Jingdong Chen, and Jacob Benesty}

% \markboth{IEEE SIGNAL PROCESSING LETTERS, VOL. XX, NO. XX, JAN 2025}
% {Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Journals}
% \maketitle

% \begin{abstract}
% The performance of deep learning-based multichannel speech enhancement methods often deteriorates when the geometric parameters of the microphone array change. Traditional approaches to mitigate this issue typically involve training on multiple microphone arrays, which can be costly. To address this challenge, we focus on uniform circular arrays and propose the use of a spatial filter bank to extract features that are approximately invariant to geometric parameters. These features are then processed by a two-stage conformer-based model (TSCBM) to enhance speech quality. Experimental results demonstrate that our proposed method can be trained on a fixed microphone array while maintaining effective performance across uniform circular arrays with unseen geometric configurations during applications. 
% \end{abstract}

% \begin{IEEEkeywords}
% Speech enhancement, multichannel processing, uniform circular microphone arrays, geometry-agnostic.
% \end{IEEEkeywords}


% \IEEEpeerreviewmaketitle
% \section{formuler}
% Consider a UCA consisting of $M$ omnidirectional sensors uniformly spaced around a circle of radius $r$.  Taking the center of the UCA as the reference point and assuming a plane wave arriving from an azimuth angle $\theta$, the phase delay at the $m$th sensor relative to the reference can be expressed as $\zeta_m \left( \omega, \theta \right) = e^{\jmath \overline{\omega} \cos \left( \theta - \psi_m \right)}$, $m = 1, 2, \ldots, M$, where $\jmath$ is the imaginary unit, $\overline{\omega} = \omega r / c$, $\omega$ is the angular frequency, and $c$ denotes the speed of sound in air. The steering vector can then be represented as
% \begin{align}
%     \label{sv}
%     \mathbf{d} \left( \omega, \theta \right)
%     & = \left[ \begin{array}{cccc}
%     \zeta_1 \left( \omega, \theta \right) & \zeta_2 \left( \omega, \theta \right) & \cdots & \zeta_M \left( \omega, \theta \right)
%     \end{array}\right]^T,
% \end{align}
% where the superscript $^T$ is the transpose operator. In the short-time-Fourier-transform (STFT) domain, the signals received by the UCA can be written as
% \begin{align}
%     \label{y-vect-def}
%     \mathbf{y} \left( k,\omega \right)
%     & = \left[ \begin{array}{cccc}
%     Y_1 \left( k, \omega \right) & Y_2 \left( k, \omega \right) & \cdots & Y_M \left( k, \omega \right)
%     \end{array} \right]^T \nonumber \\
%     & = \mathbf{x}_\mathrm{d} \left( k, \omega \right) + \mathbf{v} \left( k, \omega \right),
% \end{align}
% where $\mathbf{v} \left( k,\omega \right)$, of length $M$, is the vector of the background noise, and
% \begin{align}
%     \label{x-d-vect-def}
%     \mathbf{x}_\mathrm{d} \left( k, \omega \right)
%     & = \left[ \begin{array}{ccc}
%     X_{1, \mathrm{d}} \left( k, \omega \right) & \cdots & X_{M, \mathrm{d}} \left( k, \omega \right)
%     \end{array} \right]^T,
% \end{align}
% also of length $M$, represents the desired signal originated from the source of interest,  with 
% \begin{align}
%      X_\mathrm{m,d} \left( k, \omega \right)=G_{m,d} S(k,\omega)
% \end{align}
% $G_{m,d} \left( \omega \right)$ being the transfer function on $m$~th microphone corresponding to the direct path and early reflections,  and $S \left( k, \omega \right)$ denoting the source signal.

% The objective of this work is to estimate  the desired signal on reference point $X_\mathrm{d} \left( k, \omega \right)$ from the array observed vector $\mathbf{y} \left( k, \omega \right)$, and it can be written as
% \begin{align}
%     \label{x-d-def}
%     X_\mathrm{d} \left( k, \omega \right)
%     & = G \left( \omega \right) S \left( k, \omega \right),
% \end{align}
% where $G \left( \omega \right)$ is the transfer function on reference point corresponding to direct and early reflections.
% To accomplish this, we derive a neural network (NN) based method.
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.475\textwidth]{Fig1-ver3.pdf} 
%     \caption{The overall architecture of the proposed TSCBM+FB.}
%     \label{fig:whole}
% \end{figure}
% % \section{method}
% % \begin{align}
% %     X_{fd}(k,\omega)&=\mathbf{h}^H \mathbf{x}_{d}(k,\omega)\\
% %     &=\sum_{m=1}^{M}H_m(\omega)G_{m,d} S(k,\omega)
% % \end{align}
% \section{Method Derivation}
% \label{sec:method}

% To address the performance degradation of trained models on previously unseen arrays, we introduce a method called TSCBM+FB, which stands for two-stage conformer-based model (TSCBM) with filter bank (FB). This approach first extracts features that are independent of the array radius and the number of microphones using a spatial FB. These features are then processed and enhanced by the TSCBM. The overall architecture of this model is illustrated in Fig.~\ref{fig:whole}. In the following subsections, we detail the feature extraction process and provide a comprehensive explanation of the TSCBM architecture.

% \subsection{Spatial Feature Extraction}
% \label{ssec:SFE}

% Given the decomposition of the spatial room impulse responses, the transfer function, $G \left( \omega \right)$, is composed of the attenuation and delay corresponding to different reflection path; consequently, $G \left( \omega \right)$ can be expressed as follows:
% \begin{align}
%     \label{g-fact}
%     G \left( \omega \right)
%     & = \sum^L_{l = 1} Q_l \left( \omega \right) ,
% \end{align}
% where $Q_l \left( \omega \right)$ represents the spectrum of the impulse response corresponding to the $l$th image source with $L$ being the total number of image sources. The desired component of the source signal received by the $m$th microphone can then be written as
% \begin{align}
%     \label{x-m-d-fact}
%     X_{m, \mathrm{d}} \left( k, \omega \right)
%     & = \sum^L_{l = 1} Q_l \left( \omega \right) \zeta_m \left( \omega, \theta_l \right) S \left( k, \omega \right),
% \end{align}
% where $\zeta_m \left( \omega, \theta_l \right)$ denotes the phase delay of the $l$th path to the $m$th microphone. The vector $\mathbf{x}_\mathrm{d} \left( k, \omega \right)$ can then be expressed as
% \begin{align}
%     \label{x-d-vect-def-2}
%     \mathbf{x}_\mathrm{d} \left( k, \omega \right)
%     & = \sum^L_{l = 1} Q_l \left( \omega \right) S \left( k, \omega \right) \mathbf{d} \left( \omega, \theta_l \right).
% \end{align}
% As indicated by \eqref{x-d-vect-def-2}, changes in the UCA geometry, such as changes in the number of sensors or the radius, will affect $\mathbf{d} \left( \omega, \theta_l \right)$. This, in turn, can lead to performance degradation in deep learning models. Therefore, it is crucial to extract features that are independent of the array geometry. Specifically, a spatial filter, $\mathbf{h} \left( \omega \right)$, can be used to achieve this. Then, the filtered signal is
% \begin{align}
%     \label{z-def}
%     Z \left( k, \omega \right)
%     & = \mathbf{h}^H \left( \omega \right) \mathbf{y} \left( k, \omega \right) \nonumber \\
%     & = \mathbf{h}^H \left( \omega \right) \mathbf{x}_\mathrm{d} \left( k, \omega \right) + \mathbf{h}^H \left( \omega \right) \mathbf{v} \left( k, \omega \right) \nonumber \\
%     & = X_\mathrm{fd} \left( k, \omega \right) + V_\mathrm{rn} \left( k, \omega \right),
% \end{align}
% where the superscript $^H$ is the conjugate-transpose operator, $X_\mathrm{fd} \left( k, \omega \right)$ is the filtered desired signal, and $V_\mathrm{rn} \left( k, \omega \right)$ is the residual noise. 

% Let us examine the structure of $X_\mathrm{fd} \left( k, \omega \right)$, which is
% \begin{align}
%     \label{x-fd-def}
%     X_\mathrm{fd} \left( k, \omega \right)
%     & = \sum^L_{l = 1} Q_l \left( \omega \right) S \left( k, \omega \right) \mathbf{h}^H \left( \omega \right) \mathbf{d} \left( \omega, \theta_l \right) \nonumber \\
%     & = \sum^L_{l = 1} Q_l \left( \omega \right) S \left( k, \omega \right) \mathcal{B} \left[ \mathbf{h} \left( \omega \right), \theta_l \right],
% \end{align}
% where $\mathcal{B} \left[ \mathbf{h} \left( \omega \right), \theta_l \right]$ denotes the spatial response, i.e., the beampattern at azimuth angle $\theta_l$. 
% As shown in \eqref{x-fd-def}, $Q_l \left( \omega \right)$ and $S \left( k, \omega \right)$ are not dependent on the array geometry. If the spatial response, $\mathcal{B} \left[ \mathbf{h} \left( \omega \right), \theta_l \right]$, of the spatial filter is independent of the geometry of the UCA, then the extracted speech feature will also be independent of the geometric parameters.

% To ensure that the beampattern remains independent of the geometric parameters, we can design the filter to approximate the desired directivity pattern. To achieve this, we employ the method proposed in~\cite{huang2017design}. For a UCA, the ideal beampattern with the mainlobe directed towards $\theta_\mathrm{s}$ can be expressed as
% \begin{align}
%     \mathcal{B} \left( \mathbf{b}_{N}, \theta \right)
%     & = \sum_{n=-N}^N b_{N,n} e^{\jmath n \left( \theta - \theta_\mathrm{s} \right)} \nonumber \\
%     & = \mathbf{b}_N^T \mathbf{p} \left( \theta \right),
% \end{align}
% where $\mathbf{b}_N$ contains the coefficients determining the shape of the ideal beampattern, $N$ is the order of the beampattern, and 
% \begin{align}
%     \mathbf{p} \left( \theta \right)
%     & = \left[\begin{array}{ccccc}
%     e^{-\jmath N \theta} & \cdots & 1 & \cdots & e^{\jmath N \theta}
%     \end{array} \right]^T.
% \end{align}
% The design of the beamforming filter can be approached from a least-squares perspective \cite{huang2017design}. The filter is formulated as follows:
% \begin{align}
%     \label{h-vect-def}
%     \mathbf{h} \left( \omega \right)
%     & = \frac{1}{M} \mathbf{\Psi}^H \mathbf{J}^* \left( \overline{\omega} \right) \mathbf{\Upsilon}^* \left( \theta_{\mathrm{s}} \right) \mathbf{b}_N,
% \end{align}
% where the superscript $^*$ is the conjugate operator, and
% \begin{align}
%     \mathbf{\Psi}
%     & = \left[ \begin{array}{ccccc}
%     \boldsymbol{\psi}_{-N}^* & \cdots & \boldsymbol{\psi}_0^* & \cdots & \bm{\psi}_N^*
%     \end{array} \right]^T, \\
%     \boldsymbol{\psi}_n
%     & = \left[ \begin{array}{cccc}
%     e^{-\jmath n \psi_1} & e^{-\jmath n \psi_2} & \cdots & e^{-\jmath n \psi_M}
%     \end{array} \right]^T, \\
%     \mathbf{J} \left( \overline{\omega} \right)
%     & = \mathrm{diag} \left[ \frac{1}{\jmath^{-N}J_{-N} \left( \overline{\omega} \right)} \cdots \frac{1}{J_0 \left( \overline{\omega} \right)} \cdots \frac{1}{\jmath^N J_N \left( \overline{\omega} \right)} \right], \\
%     \mathbf{\Upsilon} \left( \theta_\mathrm{s} \right)
%     & = \mathrm{diag} \left[ e^{\jmath N \theta_\mathrm{s}} ~~\cdots~~ 1 ~~\cdots~~ e^{-\jmath N \theta_\mathrm{s}} \right],
% \end{align}
% with $J_n \left( \cdot \right)$ being the $n$th-order Bessel function of the first kind. 

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.3\textwidth]{Fig2.eps} \vskip -12pt
% \caption{Designed second-order supercardioid beampattern with varying UCA geometric parameters. Conditions: $\theta_\mathrm{s} = 0^\circ$ and $f = 4$~kHz.}
% \label{fig:beampattern1}
% \end{figure}

% Figure~\ref{fig:beampattern1} shows the beampatterns of a supercardioid beamformer designed for a UCA with different geometric parameters. The beampatterns are highly consistent, demonstrating that they remain largely unaffected by geometric variations. This consistency highlights that the features extracted using this method are primarily independent of geometric parameters, which is crucial for maintaining robustness across various array configurations.

% Although the beampattern of a spatial filter can be designed to be independent of the geometric parameters of the UCA, it mainly enhances sound from a specific direction, $\theta_\mathrm{s}$, while attenuating sound from other directions, as shown in Fig.~\ref{fig:beampattern1}. Since the speaker’s location is typically unknown in practice, it is necessary to use a set of spatial filters oriented in different directions to form a spatial FB for feature extraction. Specifically, we use a total of $I$ filters, where the $i$th filter orients toward $\theta_\mathrm{s} = \frac{i}{I} 2\pi$, and the output from this filter is denoted as $Z_i$.


% \subsection{Model Architecture}

% Our network is built upon CMGAN \cite{cao2022cmgan}, which incorporates a well-established dual-path architecture that effectively captures both temporal and frequency information in speech signals, demonstrating outstanding performance in speech enhancement tasks. To address the specific challenges we encountered, we streamlined the network structure and adapted the proposed approach to the TSCBM. It is important to highlight that our method is not limited to TSCBM and can be applied to most multichannel speech enhancement models. We choose TSCBM as the backbone model to simultaneously process multichannel signals, eliminating the need for separate processing of individual channels \cite{luo2020end, pandey2022tparn, yoshioka2022vararray}, which is crucial for reducing computational complexity.


% \subsubsection{Input Features}

% The spatial FB's output features are compressed to equalize the significance of softer sounds against louder ones:
% \begin{align} 
% Z_i^{'} = |Z_i|^c e^{\jmath \angle{Z_i}},
% \end{align}
% where $Z_i^{'}$ is the compressed feature and $c=0.3$ is the compression exponent as per \cite{cao2022cmgan}. The real and imaginary parts of $Z_i^{'}$ are concatenated to form the input $Z^{'} \in \mathcal{R}^{B \times 2I \times T \times F}$, with $T$ and $F$ representing time and frequency dimensions, respectively.

% \subsubsection{Encoder}
% The encoder maps $Z^{'}$ into a latent feature space. It initiates with a convolutional block with a kernel of $(1,1)$ and stride $(1,1)$, followed by instance normalization and PReLU activation. This yields an intermediate feature map $[B,C,T,F]$ with $C=64$. A dilated DenseNet with dilation factors of 1 and 2 is then applied. The process ends with a convolutional block with a kernel of $(1,3)$ and stride $(1,2)$, downsampling the frequency dimension.

% \subsubsection{TSCB Block}
% Intermediate features pass through two-stage conformer blocks (TSCBs) to capture temporal and frequency dependencies. Each TSCB, as shown in Fig.~\ref{fig:whole}(b), contains two conformer blocks, each addressing temporal and frequency dependencies. These blocks include two FFNNs, an MHSA mechanism with four heads, and a convolution module. Skip connections are used to preserve feature integrity.

% \subsubsection{Decoder}
% The decoder reconstructs the desired signal spectrum. It begins with a dilated DenseNet mirroring the encoder's architecture. A sub-pixel convolution block follows, doubling the feature dimension to $C=128$ and upsampling the frequency dimension via pixel shuffle. The final convolution block includes instance normalization, PReLU activation, and a kernel of $(1,2)$, yielding a final feature map with $C=2$ for the real and imaginary parts of the signal spectrum.
% \end{document}


